Separate-and-Aggregate: A Transformer-based Patch Refinement Model for Knowledge Graph Completion

Knowledge graph completion (KGC) is the task of inferencing missing facts from any given knowledge graphs (KG). Previous KGC methods typically represent knowledge graph entities and relations as trainable continuous embeddings and fuse the embeddings of the entity $h$ (or $t$) and relation $r$ into hidden representations of query $(h, r, ?)$ (or $(?, r, t$)) to approximate the missing entities. To achieve this, they either use shallow linear transformations or deep convolutional modules. However, the linear transformations suffer from the expressiveness issue while the deep convolutional modules introduce unnecessary inductive bias, which could potentially degrade the model performance. Thus, we propose a novel Transformer-based Patch Refinement Model (PatReFormer) for KGC. PatReFormer first segments the embedding into a sequence of patches and then employs cross-attention modules to allow bi-directional embedding feature interaction between the entities and relations, leading to a better understanding of the underlying KG. We conduct experiments on four popular KGC benchmarks, WN18RR, FB15k-237, YAGO37 and DB100K. The experimental results show significant performance improvement from existing KGC methods on standard KGC evaluation metrics, e.g., MRR and H@n. Our analysis first verifies the effectiveness of our model design choices in PatReFormer. We then find that PatReFormer can better capture KG information from a large relation embedding dimension. Finally, we demonstrate that the strength of PatReFormer is at complex relation types, compared to other KGC models

==> chapter/introduction.tex <==
\section{Introduction}
Knowledge graphs (KGs) have emerged as a powerful tool for representing structured knowledge in a wide range of applications, including information retrieval, question answering, recommendation systems, and natural language understanding. These graphs consist of entities, represented as nodes, and relations, represented as edges, connecting the entities. One of the primary challenges in the construction and maintenance of KGs is completing missing information, which requires predicting the tail entity given a head entity and a relation, a task known as knowledge graph completion (KGC).

Existing methods for KGC generally rely on learning embeddings for entities and relations, with the goal of capturing the inherent structure and semantics of the knowledge graph. However, these methods often fail to account for the disparity in the informativeness of relation and entity embeddings. In a typical knowledge graph, the number of relations is much less than the number of entities, resulting in relation embeddings being more informative than entity embeddings. This information imbalance can lead to suboptimal performance in KGC tasks.

To address this issue, we propose a novel approach to KGC that employs tokenized embeddings and a two-tower Transformer-like architecture. Our method is based on the assumption that relation embeddings should have larger dimensions than entity embeddings to accommodate the information disparity between them. By tokenizing the entity and relation embeddings into several patches, we aim to capture more granular information about the entities and relations while maintaining a balanced representation.

Our proposed two-tower architecture is designed to process tokenized embeddings from either entities or relations. The architecture is inspired by the Transformer model, which has achieved state-of-the-art performance in various natural language processing tasks. However, unlike the standard Transformer, our architecture does not include self-attention modules. Instead, we focus on cross-attention modules, where the attention query is generated from one tower and the key and values are from another tower. This design choice aims to promote the interaction between patches from different towers, enabling the model to better capture the relationships between entities and relations in the knowledge graph.

In addition to tokenizing embeddings, we explore the use of Locality Sensitive Hashing (LSH) for generating patches that cover different aspects of an entity or relation. LSH is a popular technique for approximate nearest neighbor search and has been widely used in various domains, including computer vision and natural language processing. In this work, we compare the performance of two LSH variants: 1) trainable LSH, where the hashing function is a trainable mapping matrix, and 2) frozen LSH, where the hashing function is a non-trainable matrix composed of a set of mutually orthogonal vectors.

To evaluate our proposed approach, we conduct experiments on several benchmark datasets for KGC tasks. Our experiments show that the tokenized embeddings combined with the two-tower architecture outperform traditional KGC methods, demonstrating the effectiveness of our approach. Furthermore, we find that the frozen LSH variant performs better than the trainable LSH variant, indicating the potential of using non-trainable hashing functions for generating patches in KGC tasks.

In summary, this paper presents a novel approach to knowledge graph completion using tokenized embeddings and a two-tower Transformer-like architecture. Our method addresses the information disparity between entity and relation embeddings in KGs and promotes the interaction between patches from different towers. Through extensive experiments, we demonstrate the superiority of our approach over traditional KGC methods and the effectiveness of frozen LSH in generating patches. 
